Deductive Optimization of Relational Data Storage

Optimizing the physical data storage and retrieval of data are two key database management problems. In this paper, we propose a language that can express a wide range of physical database layouts, going well beyond the row- and column-based methods that are widely used in database management systems. We use deductive synthesis to turn a high-level relational representation of a database query into a highly optimized low-level implementation which operates on a specialized layout of the dataset. We build a compiler for this language and conduct experiments using a popular database benchmark, which shows that the performance of these specialized queries is competitive with a state-of-the-art in memory compiled database system.

==> fig_join_elim.tex <==
\begin{figure}
  \begin{small}
    \begin{gather*}
      \inference{
        x\ \text{is fresh} &
        \partition{q}{\static{e}}{x} = (q_k, q_v) & \partition{q'}{\static{e'}}{x} = (\cdot, q_v')
      }{
        \textsf{join}(\static{e} = \static{e'}, q, q') ->
        \alist{}(\as{q_k}{x}, \ctuple{[q_v, q_v']})
      } \\
      \inference{
        x\ \text{is fresh} &
        \textsc{schema}(q) = [f_1, \dots, f_n] &
        F = \scalar{f_1}, \dots, \scalar{f_n}
      }{
        \begin{aligned}
          &\textsf{join}(e = e', q, q') -> 
          \alist{}(\as{q}{x}, \ctuple{[F, \filter{}(x.e = e', q')]})
        \end{aligned}
      } \\
      \inference{
        x, x'\ \text{is a fresh scope} & \partition{q'}{\static{e'}}{x'} = (q_k, q_v)
      }{
        \textsf{join}(e = \static{e'}, q, q') -> \textsf{depjoin}(\as{q}{x},
        \hidx{}(\as{q_k}{x'}, q_k, q_v, x.e))
      } 
    \end{gather*}
  \end{small}
  \vspace{-2ex}
  \caption{Join-elimination rules.}
  \vspace{-2ex}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> future.tex <==
\section{Future Work}

\stitle{Extensibility.} There are a wide variety of physical layouts that address
specific needs that \projname{} does not currently support. For example,
bitvectors could be added to store lists of Booleans efficiently or run-length
encoding could be used to store lists of scalars. Layouts which store tiles of
data together and allow indexing by 2D regions could be used to store spatial
data. In this work, we extend the relational algebra with a new operator for
each data structure that we introduce. This approach is sufficient when the
number of new structures is small, but is likely to become unwieldy as the
number of structures grows. An interesting area of future work is to find ways
to extend the \langname{} that increase its flexibility while still allowing
straightforward transformation rules to be written.

\stitle{Integration Into Existing DBMSs.} \Projname{} does not make any attempt
to integrate into an existing DBMS. This integration is an interesting
opportunity for future work. Modern DBMSs support materialized views, but they
are less flexible than the layouts that \projname{} supports, so \projname{}
could provide additional flexibility to the view functionality of a DBMS.


==> implang.tex <==
\section{Intermediate language}\label{sec:inter-lang}

\begin{figure}
  \begin{align*}
    Var ::=&\ \text{A variable name.} \\
    Op ::=&\ \text{An operator.} \\
    Iter ::=&\ \texttt{iter}\ Var\ (Var_1, \dots, Var_k)\{Stmt\} \\
    Stmt ::=&\ \texttt{loop} (Expr) \{Stmt\} \\
            &|\ \texttt{if} (Expr) \{ Stmt_t \}\ \texttt{else}\ \{ Stmt_f \} \\
            &|\ Stmt_1; Stmt_2 \\
            &|\ Var := Expr \\
            &|\ Var := \texttt{next}\ Var_i \\
            &|\ \texttt{init}\ Var_i\ (Expr_1, \dots, Expr_k) \\
            &|\ \texttt{yield}\ Expr \\
            &|\ \texttt{skip} \\
    Expr ::=&\ Var \\
           &|\ Integer \\
           &|\ \texttt{true}\ |\ \texttt{false} \\
           &|\ Op\ (Expr_1, \dots, Expr_k) \\
           &|\ Expr[Integer] \\
           &|\ \texttt{done}\ Var \\
    Val ::=&\ Integer \\
            &|\ \texttt{true}\ |\ \texttt{false} \\
            &|\ (Val_1, \dots, Val_k) \\
            &|\ () \\
    Type ::=&\ \texttt{int} \\
            &|\ \texttt{bool} \\
            &|\ \texttt{unit} \\
            &|\ (PType_1, \dots, PType_k)
  \end{align*}
  \caption{Syntax of the intermediate language.}
\end{figure}

\begin{figure}[h]
  \begin{align*}
    \sigma &:: Var \rightarrow Val \\
    \Sigma &:: Var \mapsto (Stmt, \sigma) \\
    S &:: Var \rightarrow ([Var], Stmt) \\
    M &:: Byte\ string
  \end{align*}
  
  \[ \inference[E-Var]{}{\langle x, \sigma\rangle \Downarrow \sigma[x]} \]
  
  \[
    \inference[E-Index]{
      \langle e, \sigma, \Sigma \rangle \Downarrow (v_1, \dots, v_k) & 1 \leq i \leq k
    }{
      \langle e[i], \sigma, \Sigma\rangle \Downarrow v_i
    }
  \]
  
  \[
    \inference[E-Done]{
      \Sigma[x] = (\_, \sigma_x)
    }{
      \langle \texttt{done}\ x, \sigma, \Sigma\rangle \Downarrow \sigma_x[done]
    }
  \]
  
  \[
    \inference[E-Read]{
      \langle e_p, \sigma, \Sigma\rangle \Downarrow p &
      \langle e_l, \sigma, \Sigma\rangle \Downarrow l & \\
      0 \leq p < |M| - l & 0 < l \leq 8
    }{
      \langle [e_p:e_l], \sigma, \Sigma\rangle  \Downarrow M[p], M[p+1], \dots, M[p+l]
    }
  \]
  
  \[
    \inference[S-Init]{
      \langle e_1, \sigma, \Sigma \rangle \Downarrow v_1 \dots
      \langle e_k, \sigma, \Sigma \rangle \Downarrow v_k & \\
      S[x'] = ([x_1, \dots, x_k], s) & \\
      \sigma' = \{ x_1 \mapsto v_1, \dots, x_k \mapsto v_k \}
    }{
      {\begin{array}{c}
         \langle \texttt{init}\ x'\ (e_1, \dots, e_k), \sigma, \Sigma \rangle
         \rightarrow \\
         \langle (), \texttt{skip}, \sigma, \Sigma[x' \mapsto (s, \sigma')] \rangle   
       \end{array}}
   }
 \]
 
  \[
    \inference[S-Yield]{
      \langle e, \sigma, \Sigma\rangle \Downarrow v
    }{
      \langle \texttt{yield}\ e, \sigma, \Sigma\rangle \rightarrow \langle v,
      \texttt{skip}, \sigma, \Sigma \rangle
    }
  \]
  
  \[
    \inference[S-Next]{
      \langle x_i, \Sigma \rangle \rightsquigarrow \langle v, \Sigma' \rangle &
      \sigma' = \sigma[x_v \mapsto v]
    }{
      \langle x_v := \texttt{next}\ x_i, \sigma, \Sigma \rangle
      \rightarrow \langle (), \texttt{skip}, \sigma', \Sigma'\rangle
    }
  \]
  
  \[
    \inference[S-Seq1]{}{
      \langle \texttt{skip}; s, \sigma, \Sigma\rangle \rightarrow \langle (),
      s, \sigma, \Sigma \rangle
    }
  \]

  \[
    \inference[S-Seq2]{
      \langle s_1, \sigma, \Sigma \rangle \rightarrow \langle v, s_1', \sigma', \Sigma' \rangle
    }{
      \langle s_1; s_2, \sigma, \Sigma \rangle \rightarrow \langle v, s_1'; s_2,
      \sigma', \Sigma' \rangle
    }
  \]
  
  \[
    \inference[S-Loop]{}{
      {\begin{array}{c}
      \langle \texttt{loop} (e) \{s\}, \sigma, \Sigma \rangle \rightarrow \\
      \langle (),
      \texttt{if}(e) \{ s; \texttt{loop} (e) \{s\} \}\{ \texttt{skip} \},
        \sigma, \Sigma \rangle
      \end{array}}
    }
  \]
  
  \[
    \inference[S-IfT]{
      \langle e, \sigma, \Sigma \rangle \Downarrow \texttt{true}
    }{
      \langle \texttt{if} (e) \{ s_t \}\ \texttt{else}\ \{ s_f \}, \sigma, \Sigma
      \rangle \rightarrow \langle (), s_t, \sigma, \Sigma \rangle
    }
  \]
  
  \[
    \inference[S-IfF]{
      \langle e, \sigma, \Sigma \rangle \Downarrow \texttt{false}
    }{
      \langle \texttt{if} (e) \{ s_t \}\ \texttt{else}\ \{ s_f \}, \sigma, \Sigma
      \rangle \rightarrow \langle (), s_f, \sigma, \Sigma \rangle
    }
  \]
  
  \[
    \inference[S-Step1]{
      \Sigma[x] = (s, \sigma) & 
      \langle s, \sigma, \Sigma\rangle \rightarrow \langle v, s', \sigma', \Sigma'\rangle &
      v \neq ()
    }{
      \langle x, \Sigma\rangle \rightsquigarrow \langle v, \Sigma'[x \mapsto (s', \sigma')] \rangle
    }
  \]
  
  \[
    \inference[S-Step2]{
      \Sigma[x] = (s, \sigma) &
      \langle s, \sigma, \Sigma\rangle \rightarrow \langle (), s', \sigma', \Sigma'\rangle & \\
      \langle x, \Sigma'[x \mapsto (s', \sigma')]\rangle \rightsquigarrow \langle v, \Sigma''\rangle
    }{
      \langle x, \Sigma\rangle \rightsquigarrow \langle v, \Sigma'' \rangle }
  \]
  \caption{Semantics of the intermediate language.}
\end{figure}

\begin{figure}[h]
  \[
    \inference[ET-Var]{x:\tau \in \Gamma}{\Gamma \vdash x : \tau}
  \]
  
  \[
    \inference[ET-Call]{
      e_f:\tau \rightarrow \tau' \in \Gamma & e_a:\tau \in \Gamma
    }{
      \Gamma \vdash e_f e_a : \tau'
    }
  \]
  
  \[
    \inference[ET-Lambda]{
      \exists \tau_1, \dots, \tau_l.\ \Gamma, x_1 : \tau_1, \dots, x_l : \tau_l \vdash S : \tau'
    }{\Gamma \vdash \lambda x_1, \dots, x_l. S : \tau \rightarrow \tau'}
  \]
  
  \[ \inference[ET-Slice]{}{\Gamma \vdash [e_p:e_l] : \texttt{bytes}} \]
  
  \[ \inference[ST-Yield]{\Gamma \vdash e : \tau}
    {\Gamma \vdash \texttt{yield}\ e : \texttt{iter}[\tau]} \]
  
  \[ \inference[ST-Next]{\exists \alpha.\ \Gamma \vdash x_f : \texttt{iter}[\alpha]}
    {\Gamma \vdash x := \texttt{next}\ x_f : \texttt{unit}} \]
  
  \[ \inference[ST-Skip]{}{\Gamma \vdash \texttt{skip} : \texttt{unit}} \]
  
  \[ \inference[ST-Seq1]{\Gamma \vdash S_1 : \texttt{unit} & \Gamma \vdash S_2 : \tau}
    {\Gamma \vdash S_1; S_2 : \tau} \]
  
  \[ \inference[ST-Seq2]{\Gamma \vdash S_1 : \tau_1 & \Gamma \vdash S_2 : \tau_2
    & \tau_1 = \tau_2}
  {\Gamma \vdash S_1; S_2 : \tau_1} \]

  \[ \inference[ST-If]{\Gamma \vdash S_t : \tau_1 & \Gamma \vdash S_f : \tau_1
    & \tau_1 = \tau_2 & \Gamma \vdash e : \texttt{bool}}
    {\Gamma \vdash \texttt{if} (e) \{ S_t \}\ \texttt{else}\ \{ S_f \} :
      \tau_1} \]
  
  \[ \inference[ST-Loop]{\Gamma \vdash S : \tau & \Gamma \vdash e : \texttt{int}}
    {\Gamma \vdash \texttt{loop} (e) \{S\} : \tau} \]
  \caption{Typing rules for the intermediate language.}
\end{figure}

% \subsection{Inlining}

% Given a program $S$ which creates, calls, then iterates through a function $f$,
% we want to create a program $S'$ which contains no call to $f$ such that $S$ and
% $S'$ are equivalent. This transformation is analogous to inlining of function
% calls, but the presence of the yield statement means that naive inlining is not
% sufficient.

% For example, consider the following program:
% \begin{align*}
%   &\texttt{fun}\ f() \{\\
%   &\quad \texttt{loop}(5) \{\ \texttt{yield}\ 0;\ \} \\
%   &\} \\
%   &\texttt{fun}\ g() \{\\
%   &\quad i := f (); \\
%   &\quad \texttt{loop}(5)\ \{ \\
%   &\quad \quad x := \texttt{next}\ i; \\
%   &\quad \quad \texttt{yield}\ x + 1; \\
%   &\quad \} \\
%   &\}
% \end{align*}
% It's clear that eliminating $f$ will be profitable and should be easy, but it's
% not clear how exactly $f$ should be removed.
% \begin{align*}
%   &\texttt{fun}\ g()\ \{\\
%   &\quad \texttt{loop}(5)\ \{ \\
%   &\quad \quad \texttt{yield}\ 1; \\
%   &\quad \} \\
%   &\}
% \end{align*}

% The key insight is that instead of inlining $f$ into its caller, we inline the
% caller into $f$.

% First, we select the fragment of $S$ where $f$ 

% \subsubsection{Correctness}


==> layout_formats.tex <==
\section{Layout Formats}\label{sec:layout-formats}
The serialization format for the layout operators is as follows:
\begin{itemize}
\item Integers are stored using the minimum number of bytes, from 1 to 8 bytes.
\item Booleans are stored as single bytes.
\item Fixed point numbers are normalized to a fixed scale, and stored as
  integers.
\item Tuples are stored as the concatenation of the layouts they contain,
  prefixed by a length.
\item Lists are stored as a length followed by the concatenation of their
  elements. They can be efficiently scanned through, but not accessed randomly
  by index.
\item Hash indexes are implemented using minimal perfect
  hashes~\cite{Botelho2007,DavideCastroReis2011}. The hash values are stored as
  in a list, but during serialization a lookup table is generated using the CMPH
  library and stored before the values. Using perfect hashing allows the hash
  indexes to have load factors up to 99\%.
\item Ordered indexes are similar to hash indexes in that they store a lookup
  table in addition to storing the values. In the case of the ordered index keys
  are stored sorted and the correct range is found by binary search.
\end{itemize}


==> unused_transforms.tex <==
\subsection{Column \& Row Stores}\label{sec:xform-col}

Storing data column-wise is efficient, because it can reduce the amount of
padding that must be added to maintain alignment. There are also a number of
data compression techniques---e.g.\ run-length encoding, delta encoding---that
work best on columnar data. However, in our layout language, manipulating
columnar data is difficult. If we represent a column store as a tuple of columns
zipped together, any transformation that changes the order of data in one column
must also update the other columns. This is straightforward if the layout is a
list of scalars, but for more complex layouts updating the column ordering is
difficult or impossible. It is convenient then to create column stores late in
the transformation process. The following rule creates a column store from a row
store:
\[
  %   \text{k is a kind, x is an expression and r is a relational expression}
  \inference{
  k = \textsf{cross} \lor k = \textsf{zip} \\
  l_1 = \alist{}(l, \textsf{scalar}(x_1)) &
  \dots &
  l_n = \alist{}(l, \textsf{scalar}(x_n))
}{
  \begin{aligned}
    &\alist{}(l, \tuple{[\textsf{scalar}(x_1), \dots, \textsf{scalar}(x_n)]}{k}) -> \\
    &\quad\ztuple{[l_1, \dots, l_n]}
  \end{aligned}
},
\]
and vice versa:
\[
  \inference{
  |l_1| = \dots = |l_n| & l = \textsf{zip}(l_1, \dots, l_n)
}{
  \begin{aligned}
    &\ztuple{[\alist{}(l_1, \textsf{scalar}(x_1)), \dots, \alist{}(l_n, \textsf{scalar}(x_n))]} -> \\
    &\quad\alist{}(l, \ctuple{[\textsf{scalar}(x_1), \dots, \textsf{scalar}(x_n)]})
  \end{aligned}
}.
\]
\todo{column store to row store needs a zip operator that we don't have rn}

\subsection{String Interning}\label{sec:xform-string}
Consider a more complex example: implementing string interning. This
transformation will replace scalars (they do not have to be strings, but strings
are a common use case) with unique identifiers, store the mapping between the
scalars and the unique ids in a hash index, and replace the ids with the
corresponding scalars when the layout is read. This transformation is valuable
when there are a small number of distinct scalar values, because each distinct
value will only be stored once.
\[
  \inference{
    q_{kv} = \textsf{select}(\{\textsf{idx}() \mapsto k, f\}, \textsf{dedup}(\textsf{select}(\{f\}, \textsf{scan}(r)))) \\
    r' = \textsf{select}(\{k\}, \textsf{join}(f = r.f, q_{kv}, \textsf{scan}(r))) \\
    q_{list} = \alist{}(\as{r'}{n}, \scalar{k}) \\
    q_{idx} = \hidx{}(\textsf{select}([\as{k}{k'}], q_{kv}), \\
    \textsf{scalar}((\select{}([f], \filter{}(k = k', q_{kv})))), k)
  }{
    \textsf{scan}(r) -> \ctuple{[q_{list}, q_{idx}]}
  }
\]
In this transformation, $f$ is a field in a relation $r$. This transformation
has four parts: (1) $l_{kv}$ relates scalars and keys. The scalars are
deduplicated before giving them a key. $\textsf{idx}()$ is a special function
that returns an auto-incrementing integer. (2) $r'$ is the relation $r$ but with
each instance of $f$ replaced by its key. (3) $l_{list}$ is a layout that
contains the values in $r'$. (4) $l_{idx}$ is a layout that contains the mapping
between the keys and the scalars, stored as a hash index. When the
\textsf{tuple} is scanned using the \textsf{cross} strategy, each key in
$l_{list}$ is used to look up the correct value in $l_{idx}$.

\subsection{Range Splitting}\label{sec:range-part}
One interesting example of a data-dependent transformation is the compression of
integers. All of our collections are homogeneous: their elements must be of the
same type. This means, for example, that if a list of integers contains one
integer which requires 64 bits to store, all of the integers will be stored in
64 bits. If most of the integers in the list are much smaller---byte sized,
say---this will waste space. If the data in the list is reordered, then the the
small integers will be stored using fewer bytes and the large integers using
more:
\[
  \inference{
    q_{lt} = \textsf{filter}(|e| < 127, q) & q_{gt} = \textsf{filter}(|e| > 127, q)
  }{
    \begin{aligned}
      &\alist{}(\as{q}{x}, \scalar{e}) -> \\
      &\quad\cctuple{[\alist{}(\as{q_{lt}}{x}, \scalar{e}), \alist{}(\as{q_{gt}}{x}, \scalar{e})]}
    \end{aligned}
  }.
\]

\subsection{Range Compression}
We can make range splitting more effective by recognizing cases where values
fall into a small range:
\[
  \inference{
    min = \min_{q} e \\
    q' = \textsf{select}(\{(e' + min) \mapsto e\}, \scalar{(e - min) \mapsto e'})
  }{
    \alist{}(\as{q}{x}, \scalar{e}) -> \alist{}(\as{q}{x}, q')
  }.
\]
Rewriting the values could allow us to use a smaller integer representation or
to apply the previous transformation. Note that this transformation depends on
the particular values stored in the layout. \projname{} can efficiently access
the data for a layout expression by generating a SQL query and using an existing
database system to execute it. We use the same mechanism when serializing a
layout.

